Hurdle-RMIL: Addressing Zero Inflation and Long-Tailed Imbalance in Infrared Rainfall Retrieval

Imbalanced labels can cause frequent samples to dominate AI-based quantitative remote sensing, degrading rare-event retrieval. In rain-rate retrieval based on satellite infrared brightness temperatures, this imbalance leads to systematic underestimation of rare high-intensity rainfall. In this study, Hurdle-Retrieval Model Imbalanced Learning (RMIL) is proposed. Following a divide-and-conquer strategy, Hurdle-RMIL separates zero inflation from the long-tailed distribution of positive rain. A hurdle model handles zero inflation, whereas RMIL exploits invariance under fixed observation conditions of the rainfall-to-satellite forward process to derive a Bayes-based transformation linking conditional distributions under naturally long-tailed and hypothetical balanced rainfall. This transformation enables the balanced-distribution model to be learned from natural samples without constructing a balanced dataset. Comparisons with conventional learning, classification-regression modeling, cost-sensitive learning, and generative learning using test data from multiple regions in China show that Hurdle-RMIL mitigates systematic underestimation and improves detection of rare high-intensity and extreme rainfall without markedly degrading lower-threshold accuracy. At 0.1-10 mm per hour, its root mean square error remains close to those of the best baselines, and it yields the highest equitable threat score (ETS) at most evaluated thresholds, with its advantage becoming more pronounced at high thresholds. At 30 mm per hour, its ETS is 0.051 versus 0.015 for the best baseline, and its mean error is -25.41 mm per hour versus -28.98 mm per hour. Case studies further show improved representations of rainfall intensity and spatial extent, demonstrating that Hurdle-RMIL effectively addresses rainfall-distribution imbalance and improves the retrieval of rare high-intensity rainfall.

==> tables/table4.tex <==

% \begin{table*}[h!tbp]
% \centering
% \begin{threeparttable} % 开始三线表环境，用于包含脚注
% \caption{Confusion matrix for graded evaluation.} 
% \label{tab:confusion_matrix}
% % \renewcommand{\arraystretch}{1.3} % 保持行高

% \begin{tabular}{lcc} % 保持三列居中对齐
%     \toprule
%     & \makecell{Obs. $\geq$ Th.} & \makecell{Obs. $<$ Th.} \\ % 使用缩写
%     \midrule
%     Ret. $\geq$ Th. & TP & FP \\ % 使用缩写
%     Ret. $<$ Th. & FN & TN \\ % 使用缩写
%     \bottomrule
% \end{tabular}

% \begin{tablenotes} % 表格脚注部分，使用小字号
%     \footnotesize 
%     % 确保在这里定义所有缩写，包括Obs., Ret., Th.
%     \item[Note:] Obs.: Observation; Ret.: Retrieval; Th.: Threshold; TP: true positive; FP: false positive; FN: false negative; TN: true negative.
% \end{tablenotes}
% \end{threeparttable}
% \end{table*}

\begin{table}[!t] % 保持单栏浮动环境 table 和顶部优先
\centering
\begin{threeparttable} % 开始三线表环境，用于包含脚注
\renewcommand{\arraystretch}{1.3} % 保持行距增加

\caption{Confusion matrix for graded evaluation.}
\label{tab:confusion_matrix}

% 移除 \footnotesize，使用文档默认字体大小
\begin{tabular}{lcc} % 保持三列
    \toprule
    & \makecell{Obs. $\geq$ Th.} & \makecell{Obs. $<$ Th.} \\ % 使用 makecell 确保对齐
    \midrule
    Ret. $\geq$ Th. & TP & FP \\
    Ret. $<$ Th. & FN & TN \\
    \bottomrule
\end{tabular}

% 增加表格内容和注释之间的垂直间距
\vspace{0.5em} % 插入额外的垂直间距

\begin{tablenotes} % 表格脚注部分
    % 移除原有的 \footnotesize
    \item[Note:] Obs.: Observation; Ret.: Retrieval; Th.: Threshold; TP: true positive; FP: false positive; FN: false negative; TN: true negative.
\end{tablenotes}
\end{threeparttable}
\end{table}
